Rankitect: Ranking Architecture Search Battling World-class Engineers at Meta Scale

Neural Architecture Search (NAS) has demonstrated its efficacy in computer vision and potential for ranking systems. However, prior work focused on academic problems, which are evaluated at small scale under well-controlled fixed baselines. In industry system, such as ranking system in Meta, it is unclear whether NAS algorithms from the literature can outperform production baselines because of: (1) scale - Meta ranking systems serve billions of users, (2) strong baselines - the baselines are production models optimized by hundreds to thousands of world-class engineers for years since the rise of deep learning, (3) dynamic baselines - engineers may have established new and stronger baselines during NAS search, and (4) efficiency - the search pipeline must yield results quickly in alignment with the productionization life cycle. In this paper, we present Rankitect, a NAS software framework for ranking systems at Meta. Rankitect seeks to build brand new architectures by composing low level building blocks from scratch. Rankitect implements and improves state-of-the-art (SOTA) NAS methods for comprehensive and fair comparison under the same search space, including sampling-based NAS, one-shot NAS, and Differentiable NAS (DNAS). We evaluate Rankitect by comparing to multiple production ranking models at Meta. We find that Rankitect can discover new models from scratch achieving competitive tradeoff between Normalized Entropy loss and FLOPs. When utilizing search space designed by engineers, Rankitect can generate better models than engineers, achieving positive offline evaluation and online A/B test at Meta scale.

==> exp_rl_slimdhen_lc_smt_bk.tex <==
\subsection{Reusing Search Space Invented by World-class Engineers}

KH: 1. SlimDHEN RL results targeting 30X; 2. LC result; 3. SMT result

we achieve much better roi when incorporate human supernet design

To search for a better ROI model for production CMF, we set up a DHEN matching SuperNN with linear operator size search only, i.e., we only search for linear operator’s size options, e.g., linear projection size, etc. There are a total of 93 linear operators that qualify for size search, each with 9 options, leading to a search space with size $9^{93}$. Our WSNAS stack is amenable to search for all block (layer) connections, different operators, and operator options (such as sizes); our primary motivation to only search for linear operator sizes in this work is to allow for an easier transfer of our search results to production. More specifically, we can identify the relevant production job config settings (such as various MLP bottleneck projection) and manually transfer our size search results. On the other hand, connection or operator change will require arch changes that are less supported. We ran our ROI-constraint search for both 4-layer DHEN (with target FLOPs 20X) and 7-layer DHEN (with target FLOPs 30X) and the results are summarized in Table 1: 
\begin{center}
\begin{tabular}{|m{9em}|m{4em}|m{4em}|m{4em}|} 
 \hline
 Supernet size \& complexity & ROI search weight & Target FLOPs & Converged FLOPs \\
 \hline\hline
 4-layer / 93-decisions & 2e-5 & 20X & 31.2X \\ 
 \hline
 4-layer / 93-decisions & 2e-4 & 20X & 20.3X \\ 
 \hline
 7-layer / 162-decisions & 2e-5 & 30X & 44.7X \\ 
 \hline
 7-layer / 162-decisions & 2e-4 & 30X & 26.3X \\ 
 \hline
\end{tabular}
\end{center}
In the end-to-end RL search, we can amortize the search cost by using the same warm-up stage for different target FLOPs/regularization weights as long as they are searching over the same search space. For example, in Table 1 the warm-up stage of 4-layer (7-layer) DHEN size only search takes about 2 (3) days and each subsequent search with different regularization weight takes about 4 (6) days. We validate the discovered two 4-layer DHEN models by retraining them from scratch and comparing them to production 18.5X and 31.3X DHEN. Figure 4 shows the training NE-gap of the discovered 20.3X 4-layer DHEN compared with CMF 10X production baseline where it achieved NE-gain of 0.06\% @60B while still trending better. In comparison, production 18.5x DHEN has flat stable 0.05\% NE-gain.
\begin{figure}[h]
\caption{TODO}
\centering
\includegraphics[width=0.48\textwidth]{Figures/wsnas_vs_10xV0.png}
\end{figure}
\begin{figure}[h]
\caption{TODO}
\centering
\includegraphics[width=0.48\textwidth]{Figures/wsnas_vs_31xDHEN.png}
\end{figure}



Next, to search for LC models with smaller FLOPs constraint, we setup a 2-layer DHEN matching SuperNN with linear operator size search only. The search space is similar to the previous one used for CMF  but with scaled down size options to accommodate smaller target FLOPs. We ran our ROI-constraint search for the 2-layer DHEN with various target FLOPs and the results are shown in Table 2:
\begin{center}
\begin{tabular}{|m{9em}|m{4em}|m{4em}|m{4em}|} 
 \hline
 Supernet size \& complexity & ROI search weight & Target FLOPs & Converged FLOPs \\
 \hline\hline
 2-layer / 28-decisions & 1e-3 & 50M & 51.8M \\ 
 \hline
 2-layer / 28-decisions & 2e-3 & 20M & 21.7M \\ 
 \hline
 2-layer / 28-decisions & 5e-3 & 12M & 11.9M \\ 
 \hline
 1-layer / 28-decisions & 1e-2 & 6M & 7.41M \\ 
 \hline
\end{tabular}
\end{center}
The warm-up stage of the above 2-layer DHEN size only search takes about 1 day and each subsequent search with different target FLOPs and regularization weight takes about 2 days. Our discovered model (first row in Table 2) has inference FLOPs 72M and achieved on-par NE compared to the best 87M model discovered by the current production AutoML searcher which is based on a random sampling approach that has O(N)-cost. A detailed comparison of our  O(1)-cost searcher with production O(N)-cost AutoML searcher is included in Table 3.
\begin{center}
\begin{tabular}{|m{10em}|m{5em}|m{5em}|} 
 \hline
 Search method & Discovered model size & Search cost (GPU-hous) \\
 \hline\hline
 WS-NAS O(1)-cost searcher & 72M & 3072 \\ 
 \hline
 Sampling based method & 87M & 25600 \\ 
 \hline
\end{tabular}
\end{center}
From Table 3, we see that our O(1)-cost searcher achieved 8.3X efficiency gain over production O(N)-cost searcher. Note that the computational cost estimation for O(1)-cost searcher in Table 3 includes the initial 24 hours of warm-up which can be shared across different searches as we did in this experiment. Compared with production O(N)-cost AutoML searcher, our O(1)-cost searcher are both more effective (discovered smaller model with on-par NE) and efficient (8.3X more TC efficient) and this leads to the selection of WS-NAS models over production AutoML models for launch proposal in Inline\_cvr\_post\_clk\_model and achieved +0.11\% pre-test GAS gain.

When applying our HPC stack ROI-constraint search to different model types, the ideal case is to conduct the search using the target model type’s data pipeline; however, this will require us to migrate/maintain a new data pipeline to HPC every time we search a new model type. In this work, we adopted the strategy of searching using the same CMF data pipeline for all model types but compressed the CMF input (dense and sparse) shape to that of the target model type. This minimizes the engineering overhead while still allowing us to apply ROI-constraint search targeting the new model type (calculating FLOPs only requires the input shape of the new model type). For example, we search for the 51.8M model in Table 2 for the LC Inline\_cvr\_post\_clk model and search for 11.9M model in Table 2 for the LC Perevent\_cvr model.
\begin{center}
\begin{tabular}{|m{10em}|m{5em}|m{5em}|} 
 \hline
 Model type & NE & FLOPs \\
 \hline\hline
 Model 1 & -0.099\% & -31.5\% \\ 
 \hline
 Model 2 & -0.053\% & -34.5\% \\ 
 \hline
 Model 3 & 0.04\% & -40\% \\ 
 \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{|m{10em}|m{5em}|m{5em}|} 
 \hline
 Model type & NE & FLOPs \\
 \hline\hline
 Model 1 & -0.254\% & +23\% \\ 
 \hline
 Model 2 & -0.173\% & +20\% \\ 
 \hline
 Model 3 & -0.25\% & +7\% \\ 
 \hline
\end{tabular}
\end{center}



\begin{table*}[t]
 \centering
\begin{tabular}{ccccccm{5em}} 
 \hline
 Model type & Supernet size \& complexity & Max size & Target size & $\alpha$ & Converged size & Search time (GPU-hour) \\
 \hline\hline
 Production CTR model & 4-layer / 93-decisions & 52.8$\times$ & 20$\times$ & 2e-5  & 31.2$\times$ & \hspace{2em}? \\ 
 \hline
  Production CTR model & 4-layer / 93-decisions & 52.8$\times$ & 20$\times$ & 2e-4 & 20.3$\times$ & \hspace{2em}? \\ 
 \hline
  Production CTR model & 7-layer / 162-decisions & ?$\times$ & 30$\times$ & 2e-5 & 44.7$\times$ & \hspace{2em}? \\ 
 \hline
  Production CTR model & 7-layer / 162-decisions & ?$\times$ & 30$\times$ & 2e-4 & 26.3$\times$ & \hspace{2em}? \\ 
 \hline
 Production CVR model-1  & 2-layer / 28-decisions & ?$\times$ & ?$\times$(50M) & 1e-3 & ?$\times$(51.8M) & \hspace{2em}? \\ 
 \hline
 Production CVR model-1 & 2-layer / 28-decisions & ?$\times$ & ?$\times$(20M) & 2e-3  & ?$\times$(21.7M) & \hspace{2em}? \\ 
 \hline
 Production CVR model-2 & 2-layer / 28-decisions & ?$\times$ & ?$\times$(12M) & 5e-3  & ?$\times$(11.9M) & \hspace{2em}? \\ 
 \hline
 Production CVR model-2 & 1-layer / 28-decisions& ?$\times$ & ?$\times$(6M) & 1e-2  & ?$\times$(7.41M) & \hspace{2em}? \\ 
 \hline
\end{tabular}
\end{table*}

==> exp_wall_clock_time_in_prod.tex <==
\subsection{Rankitect Search Time Evaluation}

Igor and KH: time and NE  comparisons of three methods

KH: LC 8.3X Efficiency versus production class AutoML

KH: transferability of models to SMT (zero cost)


==> post_supernet_training.tex <==
\subsection{Post Supernet-Training Search}

After the supernet training, a Dropout-like approach is used to randomly drop some building blocks and the rest can form the generated architectures, called subnets [1]. All subnets inherit the parameters from the supernet when evaluating their performance, e.g. normalized entropy (NE). In practice, we also use a small dataset (~300M) to fine-tune each subnet to more accurately evaluate the performance, and we call the resulting fine-tuning NE as weight sharing NE (wsNE). WsNE is highly correlated with the NE obtained by training the subnets from scratch with a large enough dataset [2, 3], which we called ground truth NE (trueNE). And as a result, we use the much cheaper wsNE to guide the search for the subnets with good trueNEs. We propose a sampling based iterative search workflow that is motivated by [TODO: add reference to current sota sampling based nas]. In summary, each iteration consists the following steps:
\begin{enumerate}
    \item We “sample (initial) random subnets” from the supernet and “obtain subnet wsNE” of these initial random models by lightweight fine-tuning; therefore, we can “add (subnet, wsNE) pairs to dataset” to get an initial dataset;
    \item We can “build a predictor of subnet wsNE” using this initial dataset. For example, we have experimented with using a simple MLP as a predictor and we believe there is pretty room to improve;
    \item Using this efficient predictor, we can randomly “sample billions of subnets” and “predict wsNE and pick subnets along Pareto front” which are fine-tuned again to “Obtain subnet wsNE” and added to the dataset. We loop again and again until wsNE saturates.
\end{enumerate}


==> rl_method_bk.tex <==
\subsubsection{One-shot NAS with Reinforcement Learning}\hfill\vspace{0.5em}

Motivated by the TuNAS work~\cite{9157751}, we also adopted reinforcement learning for efficient NAS where we treat all the decisions in our search space as independent multinomial random variables (r.v) parameterized by $\mathbf{\theta}=[\theta_i, \dots, \theta_N]$, and use REINFORCE \cite{10.1007/BF00992696} to update the sampling distribution $P_{\mathbf{\theta}}$ with policy gradient.
% Our problem formulation is similar to that of TuNAS where
% we treat all the decisions in our search space as independent multinomial random variables (r.v) parameterized by $\mathbf{\theta}=[\theta_i, \dots, \theta_N]$, and use REINFORCE \cite{10.1007/BF00992696} to update the sampling distribution $P_{\mathbf{\theta}}$ with policy gradient:
% \begin{equation}
%     \nabla_{\mathbf{\theta}} \sum_i^{T} \sum_j^{B} \log P_{\mathbf{\theta}}(a_{ij}) (R_{ij} - b),
%     \label{eq:pg_orig}
% \end{equation}
% where $a_{ij}$ is a sample of architecture selection and $R_{ij}$ is the quality (reward) of the sampled architecture $a_{ij}$. A baseline function $b$ is used to reduce the variance of policy gradient and in our work we define $b$ to be the average over all $R_{ij}$. In Eq.~\eqref{eq:pg_orig}, we aggregate over $T$ number of trainers each with $B$ batch of $(a_{ij}, B_{ij})$ examples. A unique aspect of training a industry-scale recommender model is that the training dataset consists of a single-pass of online data so that each batch of training data can also be consider as validation data. We alternate between learning the shared weights W using SGD and learning the sampling distribution $P_{\mathbf{\theta}}$ using Eq.~\eqref{eq:pg_orig}. At each step, trainer $i$ first sample a network architecture $a_{ij}$ from the current sampling distribution $P_{\mathbf{\theta}}$. Each trainer then use a single batch of training data to obtain $R_{ij}$ and update the shared weights W w.r.t the architecture $a_i$. After every trainer collected $B$ batch of $(a_{ij}, B_{ij})$ example we then use Eq.~\eqref{eq:pg_orig} to update $P_{\mathbf{\theta}}$. Every trainers update its own $P_{\mathbf{\theta}}$ using a fully synchronized policy gradient; therefore, a consistent $P_{\mathbf{\theta}}$ is maintained across all trainers at all time.
Since normalized entropy (NE) is a main optimization objective for recommender system, it is natural to consider batch-NE as a main component for $R_i$, denoted as $NE_{batch}(a_{ij})$ that is based on the evaluation of the model architecture $a_{ij}$. However, NE signal in industry-scale recommender system is: (1) extremely noisy (i.e., high variance), (2) non-stationarity distribution caused by data. We sought to reduce its variance by borrowing ideas from the control variate method where we subtract a correlated baseline reward, denoted as $NE_{baseline}$, from $NE_{batch}$. More specifically, we propose the following:
\begin{enumerate}[leftmargin=*]
    \item Represent $NE_{baseline}$ as batch-NE generated from an independently and in-place trained baseline model illustrated below (where the black and red path indicates forward and backward pass respectively):
\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{Figures/rl_baseline_reward.png}
\caption{In-place training a baseline model.}
\label{fig:rl_baseline_reward}
\end{figure}
    \item Define NE-gain ($NE\%(a_{ij})$) as the main NE signal used in on-shot NAS:
    \begin{equation}
        NE\%=\frac{NE_{batch}(a_{ij}) - NE_{baseline}}{NE_{baseline}}
        \label{eq:ne_gain}
    \end{equation}
\end{enumerate}
In practice, we are more interested in ROI-constraint search where our goal is to discover models that achieve both high performance (e.g., high CTR prediction accuracy) and low cost which is typically measured by training/deployment latency. In practice, measuring latency is difficult as it depends on the target software-hardware stack and in this work we approximate latency with model size/FLOPs. Since typically we can increase model performance by scaling up its size, the goal for ROI-constraint search thus becomes finding models that have good tradeoffs between performance vs. cost. To achieve ROI-constraint search with RL we augment the reward function with an additive cost term:
\begin{equation}
    R_{ij} = NE\%((a_{ij})) + \alpha \cdot Cost(a_{ij}),
\end{equation}
where $\alpha$ is a regularization weight that balances the trade-off between performance (NE-gain) and cost (FLOPs). Cost(a) is a cost penalty term that penalizes an RL sampled model if its FLOPs deviates from a target FLOPs, $c$ . In this work we experimented with L1 ($\|FLOPs(a_{ij})-c\|$) and ReLU ($\max(FLOPs(a_{ij})-c, \; 0)$) cost penalty function.
% \begin{align}
%     Cost(a_{ij}) & = \max(FLOPs(a_{ij})-c, \; 0) \\
%     Cost(a_{ij}) & = \|FLOPs(a_{ij})-c\|,
% \end{align}
% where $c$ is a predefined target FLOPs. 
% L1 function penalizes models with FLOPs that deviates from the targeted FLOPs both from above (too complex) and below (too simple) whereas Relu function only penalizes models that are too complex. 
From our experiment, we observe that RL search using Relu cost penalty function tends to converge to a model with smaller FLOPs and worse NE compared with those produced with using L1 cost penalty function. Our hypothesis is that the L1 cost penalty function can better guide RL search during initial exploration towards the targeted FLOPs and later lead to the convergence of a better local optimum model

REINFORCE is an on-policy method where it can only learn through sampling $(a_{ij}, R_{ij})$ from the current $P_{\mathbf{\theta}}$. In other words, a new batch of architecture $(a_{ij}$ needs to be sampled and new batch of rewards $R_{ij})$ need to be collected every time we use Eq.~\eqref{eq:pg_orig} to update $P_{\mathbf{\theta}}$. There are two challenges when applying on-policy RL methods to industry-scale recommender NAS:
\begin{enumerate}[leftmargin=*]
    \item \textbf{Costly reward evaluation:} evaluating $R_{ij})$ (such as in Eq.~\eqref{eq:ne_gain}) for a industry-scale model architecture $(a_{ij}$ is expensive, especially for an on-policy method where it can only be used once to update the policy.
    \item \textbf{Sample inefficiency:} $P_{\mathbf{\theta}}$'s updating schedule is slower than that of the supernet's shared weights due to the fact that supernet's shared weights can be updated using one sampled architecture $a_{ij}$ and one batch of training data but updating $P_{\mathbf{\theta}}$ requires a batch of $(a_{ij}, R_{ij})$ examples. For a typical industry setting, our budget for training a supernet with weight sharing is approximately 1M steps (updates). If we perform on-policy update using 100 $(a_{ij}, R_{ij})$ examples (batch-size of 100) then we are only able to perform 10K (1M/100) policy updates. The limitation on the number of policy updates together with our large search space presents a challenge for any on-policy RL algorithms.
\end{enumerate}
To address both of these challenges we adopted off-policy RL methods which allow for policy updates using $(a_{ij}, R_{ij})$ examples not sampled by the current $P_{\mathbf{\theta}}$, i.e., we can reuse past $(a_{ij}, R_{ij})$ examples with experience replay \cite{DBLP:journals/corr/MnihKSGAWR13}. This allows us to amortize the cost of $R_{ij})$ evaluation since we can reuse it multiple times to update policy. Furthermore, experience replay greatly improves sample efficiency by decoupling policy updates with supernet's shared weights updates. In this work, we followed a standard formulation of the off-policy policy gradient (PG) based on importance sampling (IS) \cite{10.5555/3020847.3020905}. A main challenge of off-policy implementation is controlling for the possible high variance (infinite variance in some cases) of the IS weights (a ratio of two probability functions). In this work, we adopted two techniques to mitigate the potential problem of high IS weights variance: (1) IS weights clipping; (2) weighted importance sampling (WIS) \cite{10.5555/3020847.3020905, 10.5555/3454287.3454448, JMLR:v21:20-124}. In summary, the policy gradient with off-policy IS is:
\begin{equation}
    \nabla_{\mathbf{\theta}} \sum_i^{T} \sum_j^{B} \frac{w_{ij}}{\sum w_{ij}} \log P_{\mathbf{\theta}}(a'_{ij}) (R'_{ij} - b'), \;\;(\mathbf{\theta}'_{ij}, a'_{ij}, R'_{ij})\sim B,
    \label{eq:pg_is}
\end{equation}
where $B$ is a replay buffer that stores past examples (note that we also need to store the multinomial r.v parameter $\mathbf{\theta}$ that are used to generate the examples), $b$ is the average over all $R'_{ij}$ and $w_{ij}$ is the WIS weights:
\begin{equation}
    \min\left[\frac{P_{\mathbf{\theta}}(a'_{ij})}{P_{\mathbf{\theta}'_{ij}}(a'_{ij}) + \epsilon}, 1e4 \right]
\end{equation}
With Eq.~\eqref{eq:pg_is} we can reuse all past sampled examples (saved in a replay buffer $B$) for training. 
% However, since RL policy is trained concurrently with the supernet training, $(a'_{ij}) (R'_{ij})$ may become obsolete if the corresponding NE based reward is calculated based on an outdated snapshot of the supernet shared weights. To address this issue, we only store $(a'_{ij}) (R'_{ij})$ sampled within a certain time window to ensure we always have “fresh” training data for RL, e.g., we only save the latest 200K samples. 
In this work we proposed a joint on-policy and off-policy policy gradient update (on/off-policy PG) where we first perform on-policy update using Eq.~\eqref{eq:pg_orig} followed by 50 off-policy updates using Eq.~\eqref{eq:pg_is}; we then store the new batch of examples from the on-policy update step to the replay buffer $B$. This gives us a 50x increase in the number of policy updates compared with on-policy REINFORCE and leads to significant faster learning.

In summary, we proposed: 1. introduce $NE\%(a_{ij})$ to reduce noise by an in-place baseline model; 2. Propose a on-policy/off-policy PG method to improve RL sample efficiency. A detailed ablation study is presented in Appendix A.

% In summary, we propose the following two improvements to RL one-shot NAS to address challenges unique to industry-scale recommender system:
% \begin{itemize}[leftmargin=*]
% \item Introduce $NE\%(a_{ij})$ to reduce noise by an in-place baseline in one-shot method.
% \item Propose a on-policy/off-policy PG method to improve RL one-shot NAS sample efficiency.
% \end{itemize}
% A detailed ablation study is presented in Appendix A to show the efficacy of the two proposals.



==> super_net_training.tex <==

\subsection{Super Net Training}

At each mini-batch, a sub-net is randomly sampled by dropping out some building operators within each choice block and connectivities in the super net, and randomly select operator dimensions. The sampled sub-net is trained for a mini-batch. In the next mini-batch, a new sub-net is randomly sampled and trained.  This iterative process repeats until the super-net and its sub-nets converge. This sub-net sampling and training strategy reduces the co-adaptation of weights across different sub-nets. However, training SuperNet to convergence is still a challenging task since the supernet is large and heterogeneous. In practice, we find the following are important for training a high qualiyt supernet:
\begin{itemize}
    \item Careful supernet warmup by training the whole net without subnet sampling for some initial steps, e.g. 200K.
    \item Designate certain percentage (e.g., 25\%) of sampled subnet to be the whole net.
    \item Design subnet sampling strategies tailored to distributed training, e.g., sampling different subnets per DDP rank.
    \item Well-tuned sampling probabilities of building operators and connections such that the properties of the sampled subnets (e.g., FLOPs, number of parameters, number of layers, etc.) are evenly distributed.
\end{itemize}

